CyberSecurity Challenges for Software Developer Awareness Training in Industrial Environments

Awareness of cybersecurity topics facilitates software developers to produce secure code. This awareness is especially important in industrial environments for the products and services in critical infrastructures. In this work, we address how to raise awareness of software developers on the topic of secure coding. We propose the "CyberSecurity Challenges", a serious game designed to be used in an industrial environment and address software developers' needs. Our work distils the experience gained in conducting these CyberSecurity Challenges in an industrial setting. The main contributions are the design of the CyberSecurity Challenges events, the analysis of the perceived benefits, and practical advice for practitioners who wish to design or refine these games.

==> tables/tbl_event_types.tex <==
%- Types of event
%    - 1) Stand-alone
%        Purpose: Raise awareness, Hiring tool, Developer Self-Assessment (e.g. further training required)
%    - 2) Workshop + CSC
%        Purpose: Practice and solidify learnt material; very good feedback
%    - 3) CSC + Workshop
%        Purpose: Adapt workshop to CSC results
\begin{spacing}{.9}
  \begin{table*}[http]
    \renewcommand{\arraystretch}{1.22}
    \scriptsize
    %\footnotesize
    %\small
    \centering
    \caption{Usage of Cybersecurity Challenges in the Industry}
    \label{tbl:csc_event_types}
    \begin{tabular}{|p{1.4cm}|p{3.2cm}|p{7.2cm}|}
        \hline
        {\bf ~~~Event} & \multirow{2}{*}{\bf ~~~~~~~Description} & \multirow{2}{*}{\bf ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~Usage} \\
        {\bf ~~~Type} & & \\
        \hline
        \hline
        Standalone
        &
        Solely CSC challenges, i.e. main event
        &
        Exercise previously acquired knowledge or acquire new knowledge, Refresher or Recruiting new staff\\
        \hline
        Workshop
        &
        The CSC is conducted after a training
        &
        Exercise acquired knowledge. Existing training is extended by one day to cover CSC\\

        \hline
        Adaptation
        &
        The CSC is conducted before a training
        &
        Collect information to adapt the focus of training
        \\
        \hline
    \end{tabular}
  \end{table*}
\end{spacing}

==> tables/tbl_pro_cons.tex <==
\begin{spacing}{.9}
  \begin{table*}[http]
    \renewcommand{\arraystretch}{1.22}
    \scriptsize
    %\footnotesize
    %\small
    \centering
    \caption{Deployment Scenarios of CyberSecurity Challenges}
    \label{tbl:csc_deployment_scenarios}
    \vspace{-1em}
    \begin{tabular}{|p{1.6cm}|p{3.2cm}|p{3.2cm}|p{3.4cm}|}
        \hline
        {\bf ~~Scenario} & {\bf ~~~~~~~Description}  & {\bf ~~~~~~~~~~~~~Pro} & {\bf ~~~~~~~~~~~~~Cons} \\
        \hline
        \hline
        \multirow{3}{1.6cm}{{\bf \vspace{0.02cm} Scenario 1}}&\multirow{3}{3.3cm}{Each participant receives a pre-prepared VM} &+ keep exercises         & - export control         \\
                         & &+ geographic distance    & - complex installation   \\
                         & &+ uniform clients/VMs    & - system hardening       \\
        \hline
        \multirow{3}{1.6cm}{{\bf \vspace{0.02cm} Scenario 2}} & \multirow{3}{3.3cm}{Players connect to a VM hosted in a server laptop or on the intranet} &+ system hardening       & - export control              \\
                         & &+ controlled environment & - limited number of clients    \\
                         & &+ no internet required   & - client might require tools   \\
        \hline
        \multirow{3}{1.6cm}{{\bf \vspace{0.02cm} Scenario 3}} & \multirow{3}{3.3cm}{Participants connect to a server deployed in the cloud}&+ scalability            & - bandwidth      \\
                         & &+ no client-side install & - hosting costs  \\
                         & &+ system hardening       & - competition experience \\
        \hline
    \end{tabular}
  \end{table*}
\end{spacing}


==> tables/tbl_survey_2.tex <==
\begin{spacing}{.7}
  \begin{table*}[http]
    \renewcommand{\arraystretch}{1.05}
    \scriptsize
    %\footnotesize
    %\small
    \centering
    \caption{Survey 2: Questions}
    \label{tbl:survey:survey_2}
    \vspace{-1em}
    \begin{tabular}{|p{0.7cm}|p{0.6cm}|p{0.75cm}|p{9.5cm}|}
        \hline
        {\bf RQ} & {\bf CT} & {\bf QID} & {\bf~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~Question} \\
        \hline
        \hline
        %%% RQ1
        \multirow{6}{0.7cm}{~RQ1} & \multirow{3}{0.6cm}{~PE} &    &  Solving challenges in the Sifu platform \underline{\hspace{1.2cm}}\\
        \cline{3-4}
        &  & Q1.2 &  ~~~~~~helps me in recognizing vulnerable code\\
        \cline{3-4}
        & & Q1.2 &  ~~~~~~helps me to understand consequences of exploiting vulnerable code\\
        \cline{2-4}
        & \multirow{2}{0.6cm}{~BE} & Q3.2 &  ~~~~~~helps me to improve my secure coding skills\\
        \cline{3-4}
        && Q4.2 &  ~~~~~~helps me to practice secure coding guidelines\\
        \cline{2-4}
        & ~PR & Q5.2 &  The Sifu platform is an adequate mean to raise awareness on secure coding\\

        %%% RQ2;   HP -> Happiness / Graziotin
        \hline
        \multirow{2}{0.7cm}{~RQ2} & \multirow{2}{0.6cm}{~~~-} & Q6.2 &  The examples in the Sifu platform are clearly presented\\
        \cline{3-4}
        && Q7.2 & My overall experience with the platform was positive \\

        \cline{1-2}\cline{3-4}
        \multirow{2}{0.7cm}{~RQ4} & \multirow{2}{0.6cm}{~HP} & Q8.2 &  It is fun to solve challenges in the Sifu platform\\
        \cline{3-4}
        && Q9.2 &  Participating in CSC makes me overall happy\\
        \hline
    \end{tabular}
    {\\\hspace{\textwidth}
                     {\scriptsize {\bf RQ}: Research Question, {\bf CT}: Construct , {\bf QID}: Question Identifier, {\bf PE}: Perception, ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ {\bf BE}: Behavior, {\bf PR}: Protection, {\bf HP}: Happiness (Graziotin et al.)}~~~~~~~~~~~~~~~~~~~~~~~~
                     }
  \end{table*}
\end{spacing}

==> tables/tbl_survey_2_rq_analysis.tex <==
\begin{spacing}{.9}
  \begin{table*}[http]
    \renewcommand{\arraystretch}{1.22}
    \scriptsize
    %\footnotesize. \multicolumn{1}{|c|}{}
    %\small
    \centering
    \caption{Analysis of Research questions for Survey 2}
    \label{tbl:survey_2:rq:analysis}
    \vspace{-1em}
    \begin{tabular}{|p{0.8cm}|p{1cm}|p{1.6cm}|p{1.6cm}|p{1.6cm}|p{1.6cm}|p{1.6cm}|}
        \hline
         & Rank & \multicolumn{1}{c|}{1} & \multicolumn{1}{|c|}{2} & \multicolumn{1}{|c|}{3} & \multicolumn{1}{|c|}{4} & \multicolumn{1}{|c|}{5} \\
        \hline
        \hline
        \multirow{2}{0.6cm}{~RQ1}  & W.Avg. & \multicolumn{1}{c|}{4.33} & \multicolumn{1}{c|}{4.00} & \multicolumn{1}{c|}{3.80} & \multicolumn{1}{c|}{3.67} & \multicolumn{1}{c|}{3.33} \\
        \cline{2-7}
        & QID & \multicolumn{1}{|c|}{Q4.2} & \multicolumn{1}{|c|}{Q3.2} & \multicolumn{1}{|c|}{Q5.2} & \multicolumn{1}{|c|}{Q1.2} & \multicolumn{1}{|c|}{Q2.2} \\
        \hline
        \hline
        \multirow{2}{0.6cm}{~RQ2}  & W.Avg. & \multicolumn{1}{|c|}{3.73} & \multicolumn{1}{|c|}{3.53} & \multicolumn{1}{|c|}{-} & \multicolumn{1}{|c|}{-} & \multicolumn{1}{|c|}{-} \\
        \cline{2-7}
        & QID & \multicolumn{1}{|c|}{Q7.2} & \multicolumn{1}{|c|}{Q6.2} & \multicolumn{1}{|c|}{-} & \multicolumn{1}{|c|}{-} & \multicolumn{1}{|c|}{-} \\
        \hline
        \hline
        \multirow{2}{0.6cm}{~RQ4}  & W.Avg. & \multicolumn{1}{|c|}{3.67} & \multicolumn{1}{|c|}{-} & \multicolumn{1}{|c|}{-} & \multicolumn{1}{|c|}{-} & \multicolumn{1}{|c|}{-}  \\
        \cline{2-7}
        & QID & \multicolumn{1}{|c|}{Q8.2, Q9.2} & \multicolumn{1}{|c|}{-} & \multicolumn{1}{|c|}{-} & \multicolumn{1}{|c|}{-} & \multicolumn{1}{|c|}{-}  \\
        \hline
    \end{tabular}
  \end{table*}
\end{spacing}
